Local Intuitionistic Modal Logics and Their Calculi

We investigate intuitionistic modal logics with locally interpreted $\square$ and $\lozenge$. The basic logic LIK is stronger than constructive modal logic WK and incomparable with intuitionistic modal logic IK. We propose an axiomatization of LIK and some of its extensions. We propose bi-nested calculi for LIK and these extensions, thus providing both a decision procedure and a procedure of finite countermodel extraction.

==> 02-calculi.tex <==
\section{Bi-nested sequent calculi}\label{sec:calculi}
 
In this section, we discuss several bi-nested calculi for these local intuitionistic logics. 
The formation of a bi-nested calculus, exploiting two kinds of nesting treating $\leq$-upper worlds and $R$-successors in the bi-relational semantics respectively, is firstly given in \cite{FIK-csl2024}. 
We begin this section by presenting a bi-nested calculus for the basic logic \dik~named \cdikk~which is tightly connected with the semantic aspect of \dik~and proven to be sound with respect to the bi-relational semantics. 
Then we show that it can be reduced to an equivalent fragment \local~by proving the admissibility of the $(\text{inter}_\downarrow)$ rule in \cdikk. We also give another calculus for \dik~which extends the calculus \cfik~given in \cite{FIK-csl2024} and is also equivalent to \cdikk. 
In addition, based on the basic calculi, sound calculi for the extensions \did~and \dit~are given as well and disjunction property for \did~and \dit~are recovered via a syntactic proof applying the calculi.

At first we list some preliminary definitions and facts held in any bi-nested calculus. 

\begin{definition}[Bi-nested sequent]\label{def-nested-sequent}
  A bi-nested sequent $S$ is defined as follows:
  \begin{itemize}
    \item  $\Rightarrow$ is a bi-nested sequent (the empty sequent);
    \item $\Gamma\Rightarrow B_1,\ldots, B_k,[S_1],\ldots,[S_m],\langle T_1\rangle,\ldots,\langle T_n\rangle$ is a bi-nested sequent if all the 
    $B_1,\ldots, B_k$ are formulas, all the $S_1,\ldots,S_m$, $T_1,\ldots, T_n$ are bi-nested sequents where $k,m,n\geq 0$, 
    and $\Gamma$ is a finite (possibly empty) multi-set of formulas.
  \end{itemize}
\end{definition}
We use $S$ and $T$ to denote a bi-nested sequent and call it simply by ``sequents" in the rest of this paper. The antecedent and succedent of a sequent $S$ are denoted by $Ant(S)$ and $Suc(S)$ respectively.

The notion of modal degree can be extended from a formula to a sequent. 

\begin{definition}[Modal degree]
  Modal degree for a formula $F$, denoted as $\textit{md}(F)$, is defined as usual. Further, let $\Gamma$ be a finite set of formulas, define $\textit{md}(\Gamma)=\textit{md}(\bigwedge \Gamma)$. 
  For a nested sequent $S$ of the following form 
  $$
  S=\Gamma\Rightarrow\Delta,[S_1],\ldots,[S_m],\langle T_1\rangle,\ldots,\langle T_n\rangle,
  $$
  define $\textit{md}(S)=$
  
  $\max\{\textit{md}(\Gamma),\textit{md}(\Delta),\textit{md}(S_1)+1,\ldots,\textit{md}(S_m)+1,\textit{md}(T_1),\ldots,\textit{md}(T_n)\}$.
\end{definition}

\begin{definition}[Context]\label{def-context}
  A context $G\{\}$ is inductively defined as follows:
  \begin{itemize}
    \item $\{\}$ is a context (the empty context). 
    \item if $\Gamma\Rightarrow\Delta$ is a sequent and  $G'\{\}$ is a context then $\Gamma\Rightarrow\Delta, \langle G'\{\}\rangle$ is a context.
    \item if $\Gamma\Rightarrow\Delta$ is a sequent and  $G'\{\}$ is a context then $\Gamma\Rightarrow\Delta, [G'\{\}]$ is a context.
    \end{itemize}
\end{definition}

\begin{example}\label{ex:context}
  Given a context $G\{\}=p\wedge q, \square r\Rightarrow \Diamond p,\langle \square p\Rightarrow [\Rightarrow q]\rangle,[\{\}]$ and a sequent $S=p\Rightarrow q\vee r,[r\Rightarrow s]$, we have $G\{S\}=p\wedge q, \square r\Rightarrow \Diamond p,\langle \square p\Rightarrow [\Rightarrow q]\rangle,[p\Rightarrow q\vee r,[r\Rightarrow s]]$. 
\end{example}

\begin{definition}
  Let \textbf{C} be a sequent calculus. The derivation relation in \textbf{C} is denoted as $\vdash_{\textbf{C}}$ and let the set of theorems $\mathbf{D}_{\mathbf{C}}=\{S~|~\vdash_{\textbf{C}}S\}$. 
  For two calculi $\mathbf{C_1}$ and $\mathbf{C_2}$, we say $\mathbf{C_1}$ is \textit{equivalent} to $\mathbf{C_2}$, abbreviated as $\mathbf{C_1}=\mathbf{C_2}$, if $\mathbf{D}_{\mathbf{C_1}}=\mathbf{D}_{\mathbf{C_2}}$. 
\end{definition}
  
\begin{proposition}\label{Prop:empty-block-derivable}
  Let $G\{\}$ be a context, $S=\Gamma\Rightarrow\Delta$ a sequent and \textbf{C}~a sequent calculus. If $\Delta$ is not $[\cdot]$-free, then $\vdash_{\textbf{C}}\Gamma\Rightarrow\Delta$ if and only if $\vdash_{\textbf{C}}\Gamma\Rightarrow\Delta,[\Rightarrow]$. 
\end{proposition}

\begin{definition}[$\flat$-operator and $\#$-operator]\label{def:star-operator}
  Let $\Lambda\Rightarrow\Theta$ be a sequent, we define $\Theta^\flat$ as follows:
  \begin{itemize}
    \item $\Theta^\flat=\emptyset$ if $\Theta$ is $[\cdot]$-free;
    \item $\Theta^\flat= [\Phi_1\Rightarrow\Psi_1^\flat], \ldots, [\Phi_k\Rightarrow\Psi_k^\flat]$, if $\Theta=\Theta_0,[\Phi_1\Rightarrow\Psi_1], \ldots, [\Phi_k\Rightarrow\Psi_k]$ and $\Theta_0$ is $[\cdot]$-free.
  \end{itemize}

  Dually, we specify the local ``negative" part of $\Lambda\Rightarrow\Theta$ by the following $\#$-operator. 
  Let $Fm(\Theta)$ the multiset of formulas directly belonging to $\Theta$. We define the $\#$-operator with annotation as follows:
  \begin{itemize}
    \item $\Rightarrow_{\Lambda\Rightarrow\Theta}\Theta^\#= \ \Rightarrow Fm(\Theta)$ if $\Theta$ is $[\cdot]$-free;
    \item $\Rightarrow_{\Lambda\Rightarrow\Theta}\Theta^\#= \ \Rightarrow Fm(\Theta_0), [\Rightarrow_{\Phi_1\Rightarrow\Psi_1}\Psi_1^\#], \ldots, [\Rightarrow_{\Phi_k\Rightarrow\Psi_k}\Psi_k^\#]$ 
    if $\Theta=\Theta_0,[\Phi_1\Rightarrow\Psi_1], \ldots, [\Phi_k\Rightarrow\Psi_k]$ and $\Theta_0$ is $[\cdot]$-free.
  \end{itemize}
\end{definition}

From the definition, given a sequent $\Lambda\Rightarrow\Theta$, we can see $\Theta^\flat$ is a multi-set of modal blocks which keeps the local ``positive" part of $\Theta$, i.e. formulas on the antecedent of nested modal blocks in $\Theta$. 
Different from the $\flat$-operator, we annotate the $\#$-sequent by the full sequent where it comes from. This will be useful in the following termination proof in Section \ref{sec:termination} when we need to recover a full sequent from an annotated $\#$-sequent. We omit the annotation, i.e. the subscript of ``$\Rightarrow$" and directly write $\Rightarrow\Theta^\#$ if we do not need to recover the full sequent. 

\begin{example}
  Consider the full sequent $G\{S\}=p\wedge q, \square r\Rightarrow \Diamond p,\langle \square p\Rightarrow [\Rightarrow q]\rangle,[p\Rightarrow q\vee r,[r\Rightarrow s]]$ which we gave got in Example \ref{ex:context}, denote $Ant(G\{S\})$ and $Suc(G\{S\})$ by $\Lambda$ and $\Theta$ respectively, we can see by definition, 
  \begin{itemize}
    \item $\Lambda\Rightarrow\Theta^\flat=p\wedge q, \square r\Rightarrow [p\Rightarrow [r\Rightarrow ]]$ while 
    \item $\Rightarrow_{\Lambda\Rightarrow\Theta}\Theta^\#= \ \Rightarrow\Diamond p,[\Rightarrow q\vee r,[\Rightarrow s]]$.
  \end{itemize}
\end{example}

Next, we present suitable bi-nested calculi for these local intuitionistic modal logics. 

\begin{definition}
  Rules for the basic logic \dik~and its modal extensions are given in Figure \ref{cdik}, which consists of the basic calculus \cdikk~and modal rules corresponding to axioms (\axiomd), ($\axiomt_\Diamond$) and ($\axiomt_\square$). 
  We define \cdid~=~\cdikk~+~(\axiomd) and \cdit~=~\cdikk~+~($\axiomt_\square$)~+~($\axiomt_\Diamond$).
\end{definition}

\begin{figure}[!htbp]
      \centering
      \small
      \noindent\fbox{
        \parbox{\linewidth}{
          {
      The basic calculus \cdikk:
      \[ 
      \AxiomC{}
      \RightLabel{\rm ($\bot_L$)}
      \UnaryInfC{$G\{\Gamma,\bot\Rightarrow\Delta\}$}
      \DisplayProof
      \qquad
      \AxiomC{}
      \RightLabel{\rm ($\top_R$)}
      \UnaryInfC{$G\{\Gamma\Rightarrow\top,\Delta\}$}
      \DisplayProof
      \qquad
      \AxiomC{}
      \RightLabel{\rm ($\text{id}$)}
      \UnaryInfC{$G\{\Gamma,A\Rightarrow\Delta,A\}$}
      \DisplayProof
      \]
      
    \[
      \AxiomC{$G\{A,B,\Gamma\Rightarrow\Delta\}$}
      \RightLabel{\rm ($\wedge_L$)}
      \UnaryInfC{$G\{A\wedge B,\Gamma\Rightarrow\Delta\}$}
      \DisplayProof
      \qquad
      \AxiomC{$G\{\Gamma\Rightarrow\Delta,A\}$}
      \AxiomC{$G\{\Gamma\Rightarrow\Delta,B\}$}
      \RightLabel{\rm ($\wedge_R$)}
      \BinaryInfC{$G\{\Gamma\Rightarrow\Delta,A\wedge B\}$}
    \DisplayProof
    \]
    
    \[
      \AxiomC{$G\{\Gamma,A\Rightarrow\Delta\}$}
      \AxiomC{$G\{\Gamma,B\Rightarrow\Delta\}$}
      \RightLabel{\rm ($\vee_L$)}
      \BinaryInfC{$G\{\Gamma,A\vee B\Rightarrow\Delta\}$}
      \DisplayProof
      \qquad
      \AxiomC{$G\{\Gamma\Rightarrow \Delta,A,B\}$}
      \RightLabel{\rm ($\vee_R$)}
      \UnaryInfC{$G\{\Gamma\Rightarrow \Delta,A\vee B\}$}
    \DisplayProof
    \]
    
    \[
    \AxiomC{$G\{\Gamma,A\supset B\Rightarrow A,\Delta\}$}
    \AxiomC{$G\{\Gamma,B\Rightarrow\Delta\}$}
    \RightLabel{\rm ($\supset_L$)}
    \BinaryInfC{$G\{\Gamma,A\supset B\Rightarrow\Delta\}$}
    \DisplayProof
    \quad
    \AxiomC{$G\{\Gamma\Rightarrow \Delta, \langle A\Rightarrow B\rangle\}$}
    \RightLabel{\rm ($\supset_R$)}
    \UnaryInfC{$G\{\Gamma\Rightarrow \Delta, A\supset B\}$}
    \DisplayProof
    \]
    
    \[
      \AxiomC{$G\{\Gamma,\square A\Rightarrow\Delta,[\Sigma,A\Rightarrow \Pi]\}$}
    \RightLabel{\rm ($\square_L$)}
    \UnaryInfC{$G\{\Gamma,\square A\Rightarrow\Delta,[\Sigma\Rightarrow \Pi]\}$}
    \DisplayProof
    \qquad
    \AxiomC{$G\{\Gamma\Rightarrow\Delta,[\Rightarrow A]\}$}
    \RightLabel{($\square_{R}$)}
    \UnaryInfC{$G\{\Gamma\Rightarrow\Delta,\square A\}$}
    \DisplayProof
    \]

    \[
      \AxiomC{$G\{\Gamma\Rightarrow\Delta,[A\Rightarrow]\}$}
      \RightLabel{\rm ($\Diamond_L$)}
      \UnaryInfC{$G\{\Gamma,\Diamond A\Rightarrow\Delta\}$}
      \DisplayProof
      \qquad
      \AxiomC{$G\{\Gamma\Rightarrow\Delta,\Diamond A,[\Sigma\Rightarrow\Pi,A]\}$}
      \RightLabel{\rm ($\Diamond_R$)}
      \UnaryInfC{$G\{\Gamma\Rightarrow\Delta,\Diamond A,[\Sigma\Rightarrow\Pi]\}$}
      \DisplayProof
    \]
    
    \[
      \AxiomC{$G\{\Gamma,\Gamma'\Rightarrow\Delta,\langle\Gamma',\Sigma\Rightarrow\Pi\rangle\}$}
      \RightLabel{\rm (\text{trans})}
      \UnaryInfC{$G\{\Gamma,\Gamma'\Rightarrow\Delta,\langle\Sigma\Rightarrow\Pi\rangle\}$}
      \DisplayProof
    \]
    
    \[
    \AxiomC{$G\{\Gamma\Rightarrow\Delta,\langle\Sigma\Rightarrow\Pi,[\Lambda\Rightarrow\Theta^\flat]\rangle,[\Lambda\Rightarrow\Theta]\}$}
    \RightLabel{$(\text{inter}_{\rightarrow})$}
    \UnaryInfC{$G\{\Gamma\Rightarrow\Delta,\langle\Sigma\Rightarrow\Pi\rangle,[\Lambda\Rightarrow\Theta]\}$}
    \DisplayProof
    \]

    \[
    \AxiomC{$G\{\Gamma\Rightarrow\Delta,\langle\Sigma\Rightarrow\Pi,[\Lambda\Rightarrow\Theta]\rangle,[\Rightarrow_{\Lambda\Rightarrow\Theta}\Theta^\#]\}$}
    \RightLabel{($\text{inter}_{\downarrow}$)}
    \UnaryInfC{$G\{\Gamma\Rightarrow\Delta,\langle\Sigma\Rightarrow\Pi, [\Lambda\Rightarrow\Theta]\rangle\}$}
    \DisplayProof
    \]

    Modal rules for the extensions:

    \[
    \AxiomC{$G\{\Gamma\Rightarrow\Delta,[\Rightarrow]\}$}
    \RightLabel{(\axiomd)}
    \UnaryInfC{$G\{\Gamma\Rightarrow\Delta\}$}
    \DisplayProof
    \]

    $$
    \begin{array}{cc}
      \AxiomC{$G\{\Gamma,\square A, A\Rightarrow\Delta\}$}
      \RightLabel{($\axiomt_\square$)}
      \UnaryInfC{$G\{\Gamma,\square A\Rightarrow\Delta\}$}
      \DisplayProof
      \quad
      \AxiomC{$G\{\Gamma\Rightarrow\Delta,\Diamond A, A\}$}
      \RightLabel{($\axiomt_\Diamond$)}
      \UnaryInfC{$G\{\Gamma\Rightarrow\Delta,\Diamond A\}$}
      \DisplayProof
    \end{array}
    $$

    }
          }
    }
    \caption{Bi-nested rules for local intuitionistic modal logics}\label{cdik}
  \end{figure}

We can verify the axiom system given in Section \ref{sec:logic} in provable in \cdikk~which can be done by showing all the axioms and rules are provable. We only give one example of the axiom (\textbf{RV}) here. 

\begin{example}
  Axiom (\textbf{RV}): $\square(p\vee q)\supset\Diamond p\vee\square q$ is provable in \cdikk. 
\end{example}
  
\begin{proof}
    To show this, it suffices to show $\square(p\vee q)\Rightarrow\Diamond p\vee\square q$ is provable. A derivation for it in \cdikk~is
    \[
      \AxiomC{}
      \RightLabel{(id)}
      \UnaryInfC{$\square(p\vee q)\Rightarrow\Diamond p,[p\Rightarrow q,p]$}
      \AxiomC{}
      \RightLabel{(id)}
      \UnaryInfC{$\square(p\vee q)\Rightarrow\Diamond p,[q\Rightarrow q,p]$}
      \RightLabel{($\vee_L$)}
      \BinaryInfC{$\square(p\vee q)\Rightarrow\Diamond p,[p\vee q\Rightarrow q,p]$}
      \RightLabel{($\square_L$)}
      \UnaryInfC{$\square(p\vee q)\Rightarrow\Diamond p,[\Rightarrow q,p]$}
      \RightLabel{($\Diamond_R$)}
      \UnaryInfC{$\square(p\vee q)\Rightarrow\Diamond p,[\Rightarrow q]$}
      \RightLabel{($\square_R$)}
      \UnaryInfC{$\square(p\vee q)\Rightarrow\Diamond p,\square q$}
      \RightLabel{($\vee_R$)}
      \UnaryInfC{$\square(p\vee q)\Rightarrow\Diamond p\vee\square q$}
      \DisplayProof
    \]
\end{proof}

And we show that \cdikk~is sound with respect to the bi-relational semantics. To reach this goal, we define the semantic interpretation of sequents and then the notion of validity. Firstly we extend the forcing relation $\Vdash$ to sequents and blocks therein. 

\begin{definition}
Let $\mathcal{M}=(W,\leq,R,V)$ be a bi-relational model and $x\in W$. The relation $\Vdash$ is extended to sequents as follows:
\begin{quote}
$\mathcal{M}, x\not\Vdash \emptyset$\\
$\mathcal{M}, x \Vdash [T]$ if for every $y$ with $Rxy$, $\mathcal{M}, y \Vdash T$\\
$\mathcal{M}, x \Vdash \langle T \rangle$ if for every $x'$ with $x\leq x'$, $\mathcal{M}, x' \Vdash T$\\
$\mathcal{M}, x \Vdash \Gamma \Rightarrow \Delta$ if either $\mathcal{M}, x \not \Vdash A$ for some $A\in \Gamma$ or $\mathcal{M}, x \Vdash {\cal O}$ for some ${\cal O} \in \Delta$
\end{quote}
We say $S$ is {\rm valid} in $\+M$ iff $\forall w\in W$, we have $\+M,w\Vdash S$. $S$ is {\rm valid} iff it is valid in every bi-relational model.
\end{definition}

Whenever the model $\mathcal{M}$ is clear, we omit it and simply write $x \Vdash {\cal O}$ for an object ${\cal O}$, which can be a formula, a sequent or a block. 
Moreover, given a sequent $S = \Gamma \Rightarrow \Delta$, we write $x \Vdash \Delta$ if there is an ${\cal O} \in \Delta$ s.t. $x \Vdash {\cal O}$ and write $x \not\Vdash \Delta$ if the condition does not hold. 

\begin{definition}
  For a rule ($r$) of the form $\frac{G\{S_1\} \quad G\{S_2\}}{G\{S\}}$ or $\frac{G\{S_1\}}{G\{S\}}$, 
  we say ($r$) is valid if $x\Vdash G\{S_i\}$ implies $x\Vdash G\{S\}$. 
\end{definition}

\begin{lemma}\label{sharp-preserving}
  Let $\Lambda\Rightarrow\Theta$ be a sequent, $\+M=(W,\leq,R,V)$ a bi-relational model and $x\in W$. If $x\Vdash \ \Rightarrow\Theta^\#$, then $x\Vdash \ \Rightarrow \Theta$.
\end{lemma}

\begin{proof}
  Induction on the structure of $\Theta$.
\end{proof}

\begin{proposition}
  ($\text{inter}_{\downarrow}$) is valid for bi-relational semantics on (DC) frames.
\end{proposition}

The validity of other rules in \cdikk~can be verified trivially and we can further obtain the soundness of this calculus. 

\begin{proposition}
  If a sequent $S$ is provable in \cdikk, then it is a validity in \dik.
\end{proposition}

Soundness for \cdid~and \cdit~can be done easily. 

Next, we consider two variants of \cdikk. First, we define 
a fragment of \cdikk~as \local~=~\cdikk$\backslash\{(\text{inter}_{\downarrow})\}$ where the $(\text{inter}_{\downarrow})$ is removed. We will show later in this section that $(\text{inter}_{\downarrow})$ is admissible in \local~and hence the fragment \local~is equivalent to the full calculus \cdikk. 

In the meantime, we can also define another calculus for \dik~from a different perspective. 
In \cite{FIK-csl2024}, \fik, which is the logic defined on the class of forward-confluent frames, is studied. Since \dik~is exactly the logic of both downward and forward-confluent frames, it can be seen as an extension of \fik~and hence we obtain the calculus \cdik~in a modular way by adding $(\text{inter}_{\downarrow})$ directly to \cfik, which is the complete calculus of \fik. 

Compared with \cdikk, the calculus \cdik~is obtained by replacing the local right-$\square$ rule by the following global one:

\[
  \AxiomC{$G\{\Gamma\Rightarrow\Delta,\langle\Rightarrow[\Rightarrow A]\rangle\}$}
  \RightLabel{($\square_{R'}$)}
  \UnaryInfC{$G\{\Gamma\Rightarrow\Delta,\square A\}$}
  \DisplayProof
\]

To be specific, we can see \cdik~=~\cdikk$\backslash \{(\square_R)\}\cup\{(\square_{R'})\}$. \footnote{By adding the corresponding modal rules to \cdik~respectively, we can also have alternative calculi for \did~and \dit~but these two calculi will not be used in the left part of the paper. }

Now we have already defined three bi-nested calculi for the basic \dik, the difference between these calculi in terms of right-$\square$ rule and $(\text{inter}_{\downarrow})$ is presented explicitly in Table \ref{dik-calculi}.

\begin{table}[!h]
  \centering
  \begin{tabular}{|c|c|c|}
    \hline
    \cdik & global $(\square_R)$ & $(\text{inter}_{\downarrow})$ \\ 
    \hline
    \cdikk & local $(\square_{R'})$ & $(\text{inter}_{\downarrow})$  \\
    \hline
    \local & local $(\square_{R'})$ &  \\
    \hline
   \end{tabular}
   \caption{Three calculi for \dik}
   \label{dik-calculi}
\end{table}

In addition, we show that all the three calculi are equivalent in the sense of provability.

Weakening and contraction rules $(w_L)(w_R)(c_L)(c_L)$ defined as usual are hp-admissible in any $\mathbf{C}\in\{$\cdikk,\local,\cdik$\}$, not only applicable to formulas but also blocks. Besides, we have the following extended weakening rules.

\begin{proposition}\label{prop:context-provability}
  Weakening rules with respect to context, $\flat$ or $\#$ operators are admissible in any $\mathbf{C}\in\{$\cdikk,\local,\cdik$\}$.

  \[
      \AxiomC{$S$}
      \RightLabel{($C_w$)}
      \UnaryInfC{$G\{S\}$}
      \DisplayProof
      \quad
      \AxiomC{$G\{\Gamma\Rightarrow\Delta^\flat\}$}
      \RightLabel{($\flat_w$)}
      \UnaryInfC{$G\{\Gamma\Rightarrow\Delta\}$}
      \DisplayProof
      \quad
      \AxiomC{$G\{\Gamma\Rightarrow\Delta^\#\}$}
      \RightLabel{($\#_w$)}
      \UnaryInfC{$G\{\Gamma\Rightarrow\Delta\}$}
      \DisplayProof
    \]
\end{proposition}

\begin{lemma}\label{lemma:local-derivable} 
  The following rule is admissible in \local.
  \[
    \AxiomC{$G\{\Gamma\Rightarrow\Delta,\langle\Sigma\Rightarrow\Pi\rangle\}$}
    \RightLabel{\text{(Loc)}}
    \UnaryInfC{$G\{\Sigma,\Gamma\Rightarrow\Delta,\Pi\}$}
    \DisplayProof
  \]
\end{lemma}

\begin{lemma}
  The downward interactive rule $(\text{inter}_{\downarrow})$ is admissible in \local. 
\end{lemma}

\begin{proposition}
   \cdik~=~\local~=~\cdikk.
\end{proposition}

The positive and negative results on the disjunction property for these local IMLs can be obtained syntactically via the bi-nested calculi defined above. In this part, for simplicity, we only work in \local~and its extensions and let \cdidd~=~\local~+~(\axiomd) and \cditt~=~\local~+~($\axiomt_\square$)~+~($\axiomt_\Diamond$).

Consider a formula $\square \bot\vee \Diamond\top$, which is provable in \local, it is easy to see that neither of its disjuncts, i.e. $\square\bot$ and $\Diamond \top$, are provable. 
With the completeness we will obtain in Section \ref{sec:completeness}, it implies that \dik~does not enjoy the disjunction property. 
However, this counterexample does not hold neither in \did~nor \dit~since $\Diamond \top$ is provable in both calculi because of the existence of (\axiomd) or ($\axiomt_\Diamond$). 
We will show in the rest of this section that the disjunction property can be recovered in both \did~and \dit. 

\begin{lemma}\label{lemma:dp-cdid}
  Suppose $S =\ \Rightarrow A_1, \ldots, A_m, \langle G_1\rangle, \ldots, \langle G_n\rangle,[H_1],\ldots,[H_l]$ is provable in \cdid, where $A_i$'s are formulas, $G_j$ and $H_k$'s are sequents. 
  Furthermore, each $H_k$ is of the form $\Rightarrow\Theta_k$ and 
  for each sequent $T\in^{[\cdot]} H_k$, $T$ has an empty antecedent. %and does not contain implication blocks on the succedent. 
  Then we claim one of the following holds in \cdid:
  \begin{itemize}
    \item there is some $i\leq m$ s.t. $\Rightarrow A_i$ is provable;
    \item there is some $j\leq n$ s.t. $\Rightarrow \langle G_j\rangle$ is provable;
    \item there is some $k\leq l$ s.t. $\Rightarrow[H_k]$ is provable.
  \end{itemize}
  %Then one of the sequents $\Rightarrow A_i, \Rightarrow \langle G_j\rangle$ and $\Rightarrow[H_k]$ is provable where $i\leq m, j\leq n$ and $k\leq l$.
\end{lemma}

By assuming the completeness of the calculus \cdidd (which we will prove also in Section \ref{sec:completeness}), we have the disjunction property for the logic \did~as a special case of the lemma above. 

\begin{proposition}[Disjunction property for \did]\label{prop:dp}
  For any formulas $A,B$, if $\Rightarrow A \lor B$ is provable in \cdidd, then either $\Rightarrow A$ or $\Rightarrow  B$ is provable.
\end{proposition}

The disjunction property also holds for \cditt~and the proof can be done similarly. 

\iffalse
The proof is almost the same as what we have done for Lemma \ref{lemma:dp-cdid}, the only different sub-case is the one when $A_1=\Diamond B$ and in the premise $B$ is provable. In \cdit, we can construct a derivation as
\[
  \AxiomC{$\Rightarrow B$}
  \RightLabel{($w_R$)}
  \UnaryInfC{$\Rightarrow B, \Diamond B$}
  \RightLabel{($\axiomt_\Diamond$)}
  \UnaryInfC{$\Rightarrow \Diamond B$}
  \DisplayProof
\]
Then we are done.
\fi

==> 03-termination.tex <==
\section{Termination}\label{sec:termination}

In this section, we will show the termination of a set-based cumulative variant of \cdikk~and then extend the termination result to corresponding calculi of the (\textbf{T}) and (\textbf{D}) extensions as well. These results will be exploited later in the next section to show that all the local intuitionistic modal logics we consider in the paper are complete with respect to the corresponding bi-relational semantics. 

The general idea of the argument is similar with the termination proof in \cite{FIK-csl2024}. We begin the section by providing a cumulative variant of \cdikk~and then define an essential relation between sequents called structural inclusion which extends the definition in \cite{FIK-csl2024} and will be useful in both termination and completeness. Based on this relation, saturation conditions will be assigned to each rule in the cumulative calculus in order to avoid redundant rule application in proof-search procedures. More essentially, the structural inclusion will be identified as the pre-order in the model construction in the completeness proof.

However, since the rule $(\text{inter}_\downarrow)$ will produce new modal blocks, we may lose some structural inclusion regarding them if we do not set any constraints on the following rule applications for these blocks. To deal with this, we need the notion of tracking record which enables us to apply rules in the way we want. 
With all the preparations done, a decision procedure for a formula in \dik~is given in the end of the section. We will also explain briefly how these results can be extended to the modal extensions \did~and \dit.

First we reform the $\#$-operator in the following way, annotating the $\#$-sequents by the full sequent where it comes from. 

\begin{definition}
  Let $Fm(\Theta)$ the multiset of formulas directly belonging to $\Theta$. We define the $\#$-operator with annotation as follows:
  \begin{itemize}
    \item $\Rightarrow_{\Lambda\Rightarrow\Theta}\Theta^\#= \ \Rightarrow Fm(\Theta)$ if $\Theta$ is $[\cdot]$-free;
    \item $\Rightarrow_{\Lambda\Rightarrow\Theta}\Theta^\#= \ \Rightarrow Fm(\Theta_0), [\Rightarrow_{\Phi_1\Rightarrow\Psi_1}\Psi_1^\#], \ldots, [\Rightarrow_{\Phi_k\Rightarrow\Psi_k}\Psi_k^\#]$ 
    if $\Theta=\Theta_0,[\Phi_1\Rightarrow\Psi_1], \ldots, [\Phi_k\Rightarrow\Psi_k]$ and $\Theta_0$ is $[\cdot]$-free.
  \end{itemize}
\end{definition}

Since $\#$-sequents only produced by ($\text{inter}_{\downarrow}$), this annotation will help us ``track" the implication block from which a $\#$-sequent 
generates. This will be useful in the following termination proof. We omit the annotation, i.e. the subscript of ``$\Rightarrow$" and directly write $\Rightarrow\Theta^\#$ if we do not need to track an  application of ($\text{inter}_{\downarrow}$).

\begin{definition}[The $\#$-annotated cumulative calculus \textbf{C}\cdikk]
  The cumulative calculus {\rm \textbf{C}\cdikk}~acts on set-based sequents, where a set-based sequent $S = \Gamma \Rightarrow \Delta$ is defined as in definition \ref{def-nested-sequent}, but $\Gamma$ is a {\em set} of formulas and $\Delta$ is a {\em set} of formulas and/or blocks (containing set-based sequents).
  The rules are as follows: 
  \begin{itemize}
    \item $(\bot_L), \ (\top_R), \ (\text{id}),\ (\square_L),\ (\Diamond_R)$, (trans) and $(\text{inter}_{\rightarrow})$ in  \cdikk. 
    \item  $(\supset_R)$ is replaced by the two rules for $A\in\Gamma$ or $A\notin\Gamma$ respectively:
    {
    \[
    \AxiomC{$G\{\Gamma\Rightarrow\Delta,A\supset B,B\}$}
    \RightLabel{\rm ($\supset_{R_1}'$)}
    \UnaryInfC{$G\{\Gamma\Rightarrow\Delta,A\supset B\}$}
    \DisplayProof
    \quad
    \AxiomC{$G\{\Gamma\Rightarrow \Delta,A\supset B,\langle A\Rightarrow B\rangle\}$}
    \RightLabel{\rm ($\supset_{R_2}'$)}
    \UnaryInfC{$G\{\Gamma\Rightarrow\Delta,A\supset B\}$}
    \DisplayProof
    \]
    }
    \item ($\text{inter}_{\downarrow}$) is replaced by the following annotated rule:
    \[
    \AxiomC{$G\{\Gamma\Rightarrow\Delta,\langle\Sigma\Rightarrow\Pi,[\Lambda\Rightarrow\Theta]\rangle,[\Rightarrow_{\Lambda\Rightarrow\Theta}\Theta^\#]\}$}
    \RightLabel{($\text{inter}'_{\downarrow}$)}
    \UnaryInfC{$G\{\Gamma\Rightarrow\Delta,\langle\Sigma\Rightarrow\Pi, [\Lambda\Rightarrow\Theta]\rangle\}$}
    \DisplayProof
    \]
    \item The other rules in \cdikk~are modified by keeping the principal formula in the premises. For example, the cumulative versions of $(\wedge_L),\ (\square_R)$ are:
    \[
      \AxiomC{$G\{A,B,A\wedge B,\Gamma\Rightarrow\Delta\}$}
    \RightLabel{\rm ($\wedge_L'$)}
    \UnaryInfC{$G\{A\wedge B,\Gamma\Rightarrow\Delta\}$}
    \DisplayProof
    \quad
    \AxiomC{$G\{\Gamma\Rightarrow\Delta,\square A,[\Rightarrow A]\}$}
    \RightLabel{\rm ($\square_R'$)}
    \UnaryInfC{$G\{\Gamma\Rightarrow\Delta,\square A\}$}
    \DisplayProof
    \]
  \end{itemize}
\end{definition}

Given the admissibility of weakening and contraction in \cdikk, the following proposition is a direct consequence.

\begin{proposition}
  A sequent $S$ is provable in \cdikk~if and only if $S$ is provable in {\rm \textbf{C}\cdikk}.
\end{proposition}

\begin{definition}[Struatural inclusion $\subseteq^\-S$]\label{def:saturation-inclusion}
  Let $S_1=\Gamma_1\Rightarrow\Delta_1,S_2=\Gamma_2\Rightarrow\Delta_2$ be two sequents. $S_1$ is said to be \textit{structurally included} in $S_2$, denoted as $S_1\subseteq^{\-S} S_2$, if all the following conditions hold:
    \begin{enumerate}
      \item[(i).] $\Gamma_1\subseteq\Gamma_2$; 
      \item[(ii).] for each $[\Lambda_1\Rightarrow\Theta_1]\in \Delta_1$, there exists $[\Lambda_2\Rightarrow\Theta_2]\in\Delta_2$ such that $\Lambda_1\Rightarrow\Theta_1\subseteq^{\-S} \Lambda_2\Rightarrow\Theta_2$;
      \item[(iii).] for each $[\Lambda_2\Rightarrow\Theta_2]\in\Delta_2$, there exists $[\Lambda_1\Rightarrow\Theta_1]\in \Delta_1$ such that $\Lambda_1\Rightarrow\Theta_1\subseteq^{\-S} \Lambda_2\Rightarrow\Theta_2$. 
    \end{enumerate}
\end{definition}

It is easy to see $\subseteq^\-S$ is both reflexive and transitive.

Then we turn to consider the saturation condition for each rule in \textbf{C}\cdikk. Since most rules in \textbf{C}\cdikk~also occur in the calculus $\mathbf{CC_{FIK}}$ given in \cite{FIK-csl2024}, the corresponding conditions remain the same, we only define the saturation condition associated with $(\square_R)$ and $(\text{inter}_\downarrow)$ here. 

\begin{definition}[Saturation condition]
  Let $S=\Gamma\Rightarrow\Delta$ be a sequent. We say $S$ satisfies the saturation condition on the top level with respect to 
  \begin{itemize}
    \item ($\Diamond_R$): If $\Diamond A\in \Delta$ and $[\Sigma\Rightarrow\Pi]\in\Delta$, then $A\in\Pi$.
    \item ($\Diamond_L$): If $\Diamond A\in\Gamma$, then there is $[\Sigma\Rightarrow\Pi]\in\Delta$ with $A\in\Sigma$.
    \item ($\square_{R}$): if $\square A\in \Delta$, then there is $[\Lambda\Rightarrow\Theta]\in\Delta$ with $A\in\Theta$.
    \item ($\square_L$): If $\square A\in\Gamma$ and $[\Sigma\Rightarrow\Pi]\in\Delta$, then $A\in \Sigma$.
    \item ($\text{inter}_{\downarrow}$): if $\langle\Sigma\Rightarrow\Pi,[\Lambda\Rightarrow\Theta]\rangle\in \Delta$, then there is $[\Phi\Rightarrow\Psi]\in\Delta$ s.t. $\Phi\Rightarrow\Psi\subseteq^{\-S}\Lambda\Rightarrow\Theta$.
    \item ($\text{inter}_{\rightarrow}$): if $\langle\Sigma\Rightarrow\Pi\rangle,[\Lambda\Rightarrow\Theta]\in\Delta$, then there is $[\Phi\Rightarrow\Psi]\in\Pi$ s.t. $\Lambda\Rightarrow\Theta\subseteq^{\-S}\Phi\Rightarrow\Psi$.
    \item ($\text{trans}$): if $\langle\Sigma\Rightarrow\Pi\rangle\in\Delta$, then $\Gamma\subseteq\Sigma$.
  \end{itemize}
  Saturation conditions for propositional rules are defined as usual.
\end{definition}

\begin{proposition}\label{sequent-inclusion}
  Let $S=\Gamma\Rightarrow\Delta$ be a sequent. If $S$ is saturated with respect to $(\text{trans})$, $(\text{inter}_{\rightarrow})$ and ($\text{inter}_{\downarrow}$), then for $\langle\Sigma\Rightarrow\Pi\rangle\in\Delta$, we have $\Gamma\Rightarrow\Delta\subseteq^\-S\Sigma\Rightarrow\Pi$.
\end{proposition}

In order to define a terminating proof-search procedure based on \textbf{C}\cdikk, as usual we set two basic constraints on the backward rule applications in order to avoid redundancy:

\indent (i)  {\em No rule is  applied to an axiom} and 

\indent (ii) {\em No rule is  applied redundantly.}

We say a backward application of a rule (R) to a sequent $S$ is {\em redundant} if $S$ already satisfies the corresponding saturation condition associated with (R).  
However, the basic constraints are not enough to restrict rule applications. First, we need the notion of ``blocking" to avoid any occurrence of loop in a derivation. 

For a sequent $S=\Gamma\Rightarrow\Delta$, let $\bar{\Delta}$ denote the $\langle\cdot\rangle$-free part of $\Delta$. 

\begin{definition}[Equivalence]\label{def:block-eq}
  Let $S_1, S_2$ be two sequents where $S_1=\Gamma_1\Rightarrow\Delta_1,S_2=\Gamma_2\Rightarrow\Delta_2$. We say $S_1$ is equivalent to $S_2$, denoted as $S_1\simeq S_2$, if $\Gamma_1=\Gamma_2$ and $\bar{\Delta_1}=\bar{\Delta_2}$.
\end{definition}

\begin{definition}[Blocked sequent]
  Given a sequent $S$ and $S_1, S_2 \in^+ S$, with   $S_1=\Gamma_1\Rightarrow\Delta_1,S_2=\Gamma_2\Rightarrow\Delta_2$. We say $S_2$ is blocked by $S_1$ in $S$, if $S_1$ is R3-saturated, $S_2\in^{\langle\cdot\rangle}S_1$ and $S_1\simeq S_2$. 
  We say that a sequent $S'$ is  {\rm blocked} in $S$ if there exists $S_1\in^+ S$ such that $S'$ is blocked by $S_1$ in $S$.
\end{definition}

Observe that if $S$ is finite, then for any $S'\in^+S$ checking whether $S'$ is  {\rm blocked} in $S$ can be effectively decided. We say $S'$ is blocked when $S$ is clear. When a sequent is blocked, it will not be expanded anymore by the proof-search procedure. An example about how this ``blocking" mechanism operates to avoid loops can be found in \cite{FIK-csl2024}.

In addition to loops, we also need to pay attention to structural inclusion since we will identify structural inclusion as the pre-order between worlds in the model construction. 
Note that what we want to obtain after proof-search is not only a saturated but also ``well-arranged" sequent in the sense that certain components of the sequent follow the structural inclusion so that we can build counterexample directly from it. In most cases, the relation we want is ensured by saturation conditions and can be obtained automatically. But when it comes to applications of $(\text{inter}_\downarrow)$, the situation is more complicated. 

\begin{example}
  Let us consider the sequent $\square(p\vee q)\Rightarrow \square r\supset\square s$. After some preliminary steps, we get two sequents:

  \begin{enumerate}
    \item[(i).] $\square(p\vee q)\Rightarrow \square r\supset\square s,\langle\square(p\vee q),\square r\Rightarrow \square s,[p\vee q,p,r\Rightarrow s]\rangle$.
    \item[(ii).] $\square(p\vee q)\Rightarrow \square r\supset\square s,\langle\square(p\vee q),\square r\Rightarrow \square s,[p\vee q,q,r\Rightarrow s]\rangle$.
  \end{enumerate}

  We select (i), continue to apply $(\text{inter}_\downarrow)$ and obtain: 
  $\square(p\vee q)\Rightarrow \square r\supset\square s,\langle\square(p\vee q),\square r\Rightarrow \square s,[p\vee q,p,r\Rightarrow s]\rangle,[\Rightarrow s]$. 
  Now, to make the new block $[\Rightarrow s]$ saturated, we need to apply further rules, and we get the following two:
  
  \begin{enumerate}
    \item[(iii).] $\square(p\vee q)\Rightarrow \square r\supset\square s,\langle\square(p\vee q),\square r\Rightarrow \square s,[p\vee q,p,r\Rightarrow s]\rangle,[p\vee q,p\Rightarrow s]$.
    \item[(iv).] $\square(p\vee q)\Rightarrow \square r\supset\square s,\langle\square(p\vee q),\square r\Rightarrow \square s,[p\vee q,p,r\Rightarrow s]\rangle,[p\vee q,q\Rightarrow s]$.
  \end{enumerate}

  As required in the model construction which will be given in the next section, we want the modal block created by $(\text{inter}_\downarrow)$ is a lower world of the one from which it is produced. By definition, in (iii), we can see $p\vee q,p\Rightarrow s\subseteq^\-S p\vee q,p,r\Rightarrow s$ but in (iv), $p\vee q,q\Rightarrow s\subsetneq^\-S p\vee q,p,r\Rightarrow s$.
\end{example}

In order to avoid this problem and maintain the structural inclusion between certain components and the modal blocks created by $(\text{inter}_\downarrow)$, we need the following mechanism in order to only focus on the suitable sequent.

\begin{definition}[Tracking record based on $\in^{[\cdot]}$]
  Let $S$ be a set-based sequent which is saturated with respect to all the left rules in {\rm \textbf{C}}\cdikk. Take an arbitrary set of formulas, denoted as $\Gamma$. 

  Let $\Omega=\{T~|~T=S~or~T\in^{[\cdot]}S\}$. 
  For each $T\in \Omega$, we define $\mathfrak{G}_S(T,\Gamma)$, the \textit{$\in^{[\cdot]}$-based tracking record} of $\Gamma$ in $S$, which is a subset of $Ant(T)$ as follows. 
  \begin{itemize}
    \item $\mathfrak{G}_S(S,\Gamma)=\Gamma\cap Ant(S)$;
    \item If $T\in^{[\cdot]}_0 T'$ for some $T'\in\Omega$, let $\mathfrak{G}_S(T,\Gamma)$ be the minimal set s.t. 
    \begin{itemize}
      \item if $\square A\in \mathfrak{G}_S(T',\Gamma)$, then $A\in\mathfrak{G}_S(T,\Gamma)$;
      \item if $\Diamond A\in \mathfrak{G}_S(T',\Gamma)$ and $A\in Ant(T)$, then $A\in\mathfrak{G}_S(T,\Gamma)$;
      \item if $A\wedge B\in \mathfrak{G}_S(T,\Gamma)$, then $A,B\in \mathfrak{G}_S(T,\Gamma)$;
      \item if $A\vee B\in \mathfrak{G}_S(T,\Gamma)$ and $A\in Ant(T)$(resp. $B\in Ant(T)$), then $A\in \mathfrak{G}_S(T,\Gamma)$(resp. $B\in \mathfrak{G}_S(T,\Gamma)$);
      \item if $A\supset B\in \mathfrak{G}_S(T,\Gamma)$ and $B\in Ant(T)$, then $B\in \mathfrak{G}_S(T,\Gamma)$.
    \end{itemize}
  \end{itemize}  
\end{definition}

With the notion of tracking record, we propose the realization procedure for certain blocks in a sequent as below.

\begin{definition}[Realization procedure]\label{def:realization}
  Let $S=\Gamma\Rightarrow\Delta,\langle S_1\rangle,[S_2]$, where $S_1=\Sigma\Rightarrow\Pi,[\Lambda\Rightarrow\Theta]$, $S_2= \ \Rightarrow_{\Lambda\Rightarrow\Theta}\Theta^\#$ and $\Gamma\subseteq\Sigma$. 
  Besides, $S_1$ is saturated with respect to all the left rules in {\rm \textbf{C}\cdikk}. 
  Based on the $\in^{[\cdot]}$-based tracking record of $\Gamma$ in $S_1$, we define the \textit{realization procedure} for the block $[S_2]$ in $S$. 
  \begin{enumerate}
    \item[(i).] First for each $T\in^+ S_2$, define the realization function $f_{S_1}(T)$.
    %or $f(T)$ for short when $S_1$ is clear. 
    
    \noindent By definition, $T$ is of the form $\Rightarrow_{\Phi\Rightarrow\Psi}\Psi^\#$ for some $\Phi\Rightarrow\Psi\in^+\Lambda\Rightarrow\Theta$. $f_{S_1}(T)$ is defined inductively on the structure of $\Psi^\#$ as follows. 

    \begin{itemize}
      \item if $\Psi^\#$ is block-free, then $f_{S_1}(T)=\mathfrak{G}(\Phi\Rightarrow\Psi,\Gamma)\Rightarrow\Psi^\#$.
      \item otherwise $\Psi^\#= \Psi_0, [T_1], \ldots, [T_k]$ where $\Psi_0$ is a set of formulas, then 
      $f_{S_1}(T)=\mathfrak{G}(\Phi\Rightarrow\Psi,\Gamma)\Rightarrow \Psi_0, [f_{S_1}(T_1)], \ldots, [f_{S_1}(T_k)]$.
    \end{itemize}
    \item[(ii).] Then by the realization function, we obtain the realization of $S_2$, which is $f_{S_1}(S_2)$.
    \item[(iii).] As a result, the entire sequent is $\Gamma\Rightarrow\Delta,\langle S_1\rangle,[f_{S_1}(S_2)]$. 
  \end{enumerate}
\end{definition}

The following proposition says what we obtain by the realization procedure described above is a saturated sequent which meets our requirement on the structural inclusion between certain blocks. Also, the same sequent can be obtained by applying certain rules in the calculus as well.  

\begin{proposition}\label{prop:realization}
  Let $S=\Gamma\Rightarrow\Delta,\langle S_1\rangle,[S_2]$, where $S_1=\Sigma\Rightarrow\Pi,[\Lambda\Rightarrow\Theta]$ and $S_2= \ \Rightarrow_{\Lambda\Rightarrow\Theta}\Theta^\#$ and $\Gamma\subseteq\Sigma$. 

  If $S_1$ is saturated with respect to all the left rules in {\rm \textbf{C}}\cdikk, then for the sequent $S'=\Gamma\Rightarrow\Delta,\langle S_1\rangle,[f_{S_1}(S_2)]$ which is obtained by the realization procedure in Definition \ref{def:realization}, we have
  \begin{enumerate}
    \item[(i).] $S'$ is saturated with respect to all the left rules regarding or within $[f_{S_1}(S_2)]$;
    \item[(ii).] $f_{S_1}(S_2)\subseteq^\-S \Lambda\Rightarrow\Theta$;
    \item[(iii).] $S'$ can be obtained by applying left rules in {\rm \textbf{C}}\cdikk~to $[S_2]$ in $S$ in finite steps.
  \end{enumerate}
\end{proposition}

Now we turn to provide the proof-search procedure, we first divide rules of \textbf{C}\cdikk~into four groups and define different levels of saturation.
\begin{enumerate}
  \item[(R1)] basic rules: all propositional and modal rules except $(\supset_R)$;
  \item[(R2)] rules that transfer formulas and blocks into an implication block: (trans) and $\text{(inter)}_{\rightarrow}$;
  \item[(R3)] rules that create implication blocks: $(\supset_R)$;
  \item[(R4)] rule that transfers blocks out of an implication block: $\text{(inter)}_{\downarrow}$.
\end{enumerate}

%Compared with the classification on rules in $\textbf{CC}_{\textbf{FIK}}$, we see the local right rule for $\square$ is moved to the R1 group, and R4, which consists of $\text{(inter)}_{\downarrow}$ only, will be treated specially in the following proof-search procedures we propose.

\begin{definition}[Saturation]\label{3-saturation}
  Let $S =\Gamma\Rightarrow\Delta$ be a sequent and not an axiom. $S$ is called: 
  \begin{itemize}
    \item {\rm R1-saturated} if $\Gamma\Rightarrow\bar{\Delta}$ satisfies all the saturation conditions of R1 rules;
    \item {\rm R2-saturated} if $S$ is R1-saturated and $S$ satisfies saturation conditions of R2 rules for blocks $\langle S_1\rangle,[S_2]$ s.t. $S_1 \in^{\langle\cdot\rangle}_0 S$ and $S_2 \in^{[\cdot]}_0 S$;
    \item {\rm R3-saturated} if $S$ is R2-saturated and $S$ satisfies saturation conditions of R3 rules for formulas $A\supset B\in \Delta$;
    \item {\rm R4-saturated} $S$ is R3-saturated and $S$ satisfies saturation conditions of R4 rule for each implication block $\langle\Sigma\Rightarrow\Pi,[S_1]\rangle$ s.t. $\Sigma\Rightarrow\Pi,[S_1]\in^{\langle\cdot\rangle}_0 S$.
  \end{itemize}
\end{definition}

\begin{definition}[Global saturation]
  Let $S$ be a sequent and not an axiom. $S$ is called:
  \begin{itemize}
    \item {\rm global-Ri-saturated} if for each $T\in^+S$, $T$ is either Ri-saturated or blocked, where $i\in\{1,2,3\}$;
    \item {\rm global-saturated} if for each $T\in^+S$, $T$ is either R4-saturated or blocked.
  \end{itemize}
\end{definition}

In order to specify the proof-search procedure, we make use of the following four macro-procedures that extend a given derivation $\+D$ by expanding a leaf $S$. Each procedure applies rules {\em non-redundantly} to some $T=\Gamma\Rightarrow\Delta\in^+S$, that we recall it means that $S = G\{T\}$ for some context $G$.
\begin{itemize}
  \item $\textbf{EXP1}(\+D, S, T)= \+D'$ where $\+D'$ is the extension of $\+D$  obtained by applying  R1 rules to every formula in $\Gamma\Rightarrow\bar{\Delta}$. 
  \item $\textbf{EXP2}(\+D, S, T)= \+D'$ where $\+D'$ is the extension of $\+D$  obtained by applying R2-rules to blocks $\langle T_i\rangle,[T_j]\in\Delta$. 
  \item $\textbf{EXP3}(\+D, S, T)= \+D'$ where $\+D'$ is the extension of $\+D$  obtained by applying R3-rules to formulas $A\supset B\in\Delta$. 
  \item  $\textbf{EXP4}(\+D, S, T)= \+D'$ where $\+D'$ is the extension of $\+D$  obtained by applying (i) R4-rule to each implication block $T'\in^+T$ and (ii) realization procedures to modal blocks produced in (i).
\end{itemize}

It is easy to see all of these four macro-steps terminates.

\begin{proposition}\label{prop:expi-terminates}
  Given a finite derivation $\+D$, a finite leaf $S$ of $\+D$ and $T\in^+S$, then for $i\in\{1,2,3,4\}$, each $\textbf{EXPi}(\+D, S, T)$ terminates by producing a finite expansion of $\+D$ where all sequents are finite. 
\end{proposition}

With the macro-steps given above, we give the following preliminary procedure based on $\textbf{EXP1}(\cdot)$ to $\textbf{EXP3}(\cdot)$, denoted as $\text{PROCEDURE}_0(\+D)$, where $\+D$ is a finite derivation. See Algorithm \ref{PROCEDURE0}. Then based on $\text{PROCEDURE}_0(\cdot)$, the proof-search procedure $\text{PROCEDURE}(A)$ for a formula $A$ in \dik~is given as below. See Algorithm \ref{PROCEDURE}.

\begin{algorithm}[!htb]
  \caption{$\text{PROCEDURE}_0(\+D)$}\label{PROCEDURE0}
  \KwIn{$\+D$}
  initialization $\+D=\+D_0$\;
    \Repeat{FALSE}{
      \uIf{all the leaves of $\+D$ are axiomatic}{
        return ``PROVABLE" and $\+D$ }
      \uElseIf{there is a non-axiomatic leaf of $\+D$ which is global-R3-saturated}{return $\+D$} 
    \Else{{\bf select} one non-axiomatic leaf $S$ of $\+D$ that is not global-R3-saturated\\
         { \uIf{ $S$ is global-R2-saturated}{{\bf for} all $T\in^+S$ such that $T$ is a $\in^{\langle\cdot\rangle}$-minimal and not R3-saturated, check whether $T$ is blocked in $S$, if not, let  $\+D = \textbf{EXP3}(\+D, S, T)$}
        \uElseIf{ if  $S$ is global-R1-saturated}
            {{\bf for} all  $T\in^+ S$ that is not R2-saturated, let $\+D = \textbf{EXP2}(\+D, S, T)$}
         \uElse{{\bf for} all  $T\in^+ S$ that is not R1-saturated, let $\+D = \textbf{EXP1}(\+D, S, T)$}
          }
        }
    }
\end{algorithm}

\iffalse
\begin{algorithm}[!htb] % enter the algorithm environment
  \caption{$\text{PROCEDURE}_0(\+D)$}
  \begin{algorithmic}[1]
    \STATE \textbf{Input} $\+D$
    %\STATE \textbf{Initialization} $\+D=\+D_0$
      \IF{all the leaves of $\+D$ are axiomatic}
          \STATE return ``PROVABLE" and $\+D$
      \ELSE
          \IF{there is a non-axiomatic leaf of $\+D$ that is global-R3-saturated}
            \STATE return $\+D$
          \ELSE 
            \STATE select one non-axiomatic leaf $S$ of $\+D$ that is not global-R3-saturated
            \IF{$S$ is global-R2-saturated}
              \STATE {\bf for} all $T\in^+S$ such that $T$ is a $\in^{\langle\cdot\rangle}$-minimal and not R3-saturated, check whether $T$ is blocked in $S$, if not, let  $\+D = \textbf{EXP3}(\+D, S, T)$
            \ELSE 
              \IF{$S$ is global-R1-saturated}
                \STATE {\bf for} all  $T\in^+ S$ that is not R2-saturated, let $\+D = \textbf{EXP2}(\+D, S, T)$
              \ELSE 
                \STATE {\bf for} all  $T\in^+ S$ that is not R1-saturated, let $\+D = \textbf{EXP1}(\+D, S, T)$
              \ENDIF 
            \ENDIF 
          \ENDIF  
      \ENDIF
  \end{algorithmic}
\end{algorithm}
\fi

\begin{algorithm}[!htb]
  \caption{$\text{PROCEDURE}(A)$}\label{PROCEDURE}
  \KwIn{$\+D_0=\ \Rightarrow A$}
  initialization $\+D=\+D_0$\;
    \Repeat{FALSE}{
      \uIf{all the leaves of $\+D$ are axiomatic}{
        return ``PROVABLE" and $\+D$ }
      \uElseIf{ther is a non-axiomatic leaf of $\+D$ which is global-saturated}{return  ``UNPROVABLE" and $\+D$} 
    \Else{
         { \uIf{select one non-axiomatic leaf $S$ of $\+D$ which is global-R3-saturated}{{\bf for} all $T\in^+S$, let $\+D =\textbf{EXP4}(\+D, S, T)$\\
         }
        \Else{$\text{PROCEDURE}_0(\+D)$}
          }
        }
    }
\end{algorithm}

\iffalse
\begin{algorithm}[!htb] 
  \caption{$\text{PROCEDURE}(A)$}
  \begin{algorithmic}[1]
      \STATE \textbf{Input} $\+D_0=\ \Rightarrow A$
      \STATE \textbf{Initialization} $\+D=\+D_0$
      \IF{all the leaves of $\+D$ are axiomatic}
          \STATE return ``PROVABLE" and $\+D$
      \ELSE
        \IF{there is a non-axiomatic leaf $S$ of $\+D$ that is global-R3-saturated}
        \STATE {\bf for} all $T\in^+S$, let $\+D =\textbf{EXP4}(\+D, S, T)$
        \ELSE 
        \STATE $\text{PROCEDURE}_0(\+D)$
        \ENDIF
      \ENDIF
  \end{algorithmic}
\end{algorithm}
\fi

\begin{remark}
  We give some remarks on the mechanism of $\text{PROCEDURE}(A)$. 
  \begin{itemize}
    \item Given a formula $A$, following this proof-search algorithm, we obtain a derivation $\+D$ where each leaf $S$ is either an axiom or global-saturated. And we can see $(\text{inter}_{\downarrow})$ is not considered in $\text{PROCEDURE}_0(\cdot)$ where only rules from \local~are applied. Since we already show that ($\text{inter}_{\downarrow}$) is admissible in \local, it means if $A$ is provable, then the proof is constructed in the first round of $\text{PROCEDURE}_0(\cdot)$, namely $\text{PROCEDURE}_0(\Rightarrow A)$.
    \item Loop between $(\text{inter}_{\downarrow})$ and $(\text{inter}_{\rightarrow})$ is prevented by the saturation conditions.
    Consider a sequent $S=\Gamma\Rightarrow\Delta,\langle\Sigma\Rightarrow\Pi\rangle,[\Lambda\Rightarrow\Theta]$. If the blocks $\langle\Sigma\Rightarrow\Pi\rangle,[\Lambda\Rightarrow\Theta]$ already saturated with $(\text{inter}_{\rightarrow})$, then there is some $[\Phi\Rightarrow\Psi]\in \Pi$ s.t. $\Lambda\Rightarrow\Theta \subseteq^\-S\Phi\Rightarrow\Psi$. In the meantime, the saturation condition of $(\text{inter}_{\downarrow})$ for the implication block $\langle\Sigma\Rightarrow\Pi',[\Phi\Rightarrow\Psi]\rangle$ is satisfied as well. Thus it is unnecessary to apply $(\text{inter}_{\downarrow})$ to the block and then produce another modal block $[\Rightarrow \Psi^\#]$ any more. The other direction is similar.
    \item Structural inclusion in Proposition \ref{prop:realization} (ii) is preserved. Consider a global-R3-saturated sequent $S=\Gamma\Rightarrow\Delta,\langle \Sigma\Rightarrow\Pi,[S_1]\rangle,[S_2]$ where $S_2$ is produced by applying $(\text{inter}_{\downarrow})$ to $S_1$ and $S_2\subseteq^\-S S_1$. We claim in all the following stages, $S_1$ will be unchanged and for any $S_2'$ expanding $S_1$, we still have $S_2'\subseteq^\-S S_1$. The invariance of $S_1$ is trivial since it is already global-R3-saturated and according to the algorithm, no other formulas can be introduced into the block $[S_1]$ in the following steps. For $S_2$, it may go into some further rounds of $\text{PROCEDURE}_0(\cdot)$, but all the left rules will only be applied inside new implication blocks created in $S_2$. While for the $\langle\cdot\rangle$-free part of $S_2$, it is already saturated with all the left rules due to the realization procedure and hence will remain the same in the following process. Thus, though $S_2$ may be extended to some $S_2'$, it still holds that $S_2'\subseteq^\-S S_1$.
  \end{itemize}
\end{remark}

Lastly, we show that $\text{PROCEDURE}(A)$ terminates. 

\begin{proposition}\label{prop:md-preserve}
  Let $(r)$ be a rule in \textbf{C}\cdikk~and of one of the following forms,
  \[
      \AxiomC{$S_0$}
      \RightLabel{($r$)}
      \UnaryInfC{$S$}
      \DisplayProof
      \quad
      \AxiomC{$S_1$}
      \AxiomC{$S_2$}
      \RightLabel{($r$)}
      \BinaryInfC{$S$}
      \DisplayProof
    \]
  If $md(S)=k$, then in both cases, the modal degree of the premise(s) remains the same, i.e. $md(S_0)=md(S_1)=md(S_2)=k$.
\end{proposition}

\begin{proof}
  By checking all the rules in \textbf{C}\cdikk~one by one.
\end{proof}

\begin{theorem}[Termination for \textbf{C}\cdikk]\label{termination}
  Let $A$ be a formula. Proof-search for the sequent $\Rightarrow A$ in {\rm \textbf{C}}\cdikk~terminates with a finite derivation in which either all the leaves are axiomatic or there is at least one global-saturated leaf.
\end{theorem}

Similarly as what we have done above for \dik, we exploit cumulative variants of \cdid~and \cdit~to show termination. 
The cumulative version of \cdid, denoted by \textbf{C}\cdid, is defined as \textbf{C}\cdikk~plus the cumulative version of (\axiomd) and \textbf{C}\dit~for cumulative \cdit~is defined in the same way. 
Meanwhile, we define saturation conditions for (\axiomd), ($\axiomt_\square$) and ($\axiomt_\Diamond$) as below.

\begin{definition}
  Let $S=\Gamma\Rightarrow\Delta$ be a sequent. We say $S$ satisfies the saturation condition \textit{on the top level} w.r.t 
  \begin{itemize}
    \item (\axiomd): if $\Gamma^\square\cup\Delta^\Diamond$ is non-empty, then $\Delta$ is not $[\cdot]$-free.
    \item ($\axiomt_\square$): if $\square A\in \Gamma$, then $A\in\Gamma$.
    \item ($\axiomt_\Diamond$): if $\Diamond A\in\Delta$, then $A\in\Delta$.
  \end{itemize}
\end{definition}

Note that from a backward direction (\axiomd) creates an empty modal block on the succedent of the premise, if there is no constraint, we can continue to apply (\axiomd) to the empty sequent within the empty modal block. This process would not terminate and would result in infinite empty structures. The saturation condition for (\axiomd) effectively avoids this situation. For example, for a simple sequent $p\Rightarrow q$, since there is no modal formula in it, it satisfies the saturation condition for (\axiomd) automatically and we do not need to apply (\axiomd) and add useless $[\cdot]$ blocks to a sequent. 

As for the procedure, we treat the rules of (\axiomd) and (\axiomt)'s differently. As extra steps in $\mathrm{PROCEDURE}_0$ (see Algorithm \ref{PROCEDURE0}), the rule (\axiomd) is applied immediately after each round of $\textbf{EXP2}(\cdot)$ while the two (\axiomt) rules are regarded as part of the basic rules and applied within $\textbf{EXP1}(\cdot)$ together with other logical rules. Different levels of saturation in \textbf{C}\cdid~and \textbf{C}\cdit~are then adjusted accordingly. Termination for the procedures of both \textbf{C}\cdid~and \textbf{C}\cdit~are direct. Following the same proof for \textbf{C}\cdikk, we can obtain termination of proof-search in these two calculi as well.

\begin{theorem}[Termination for {\rm \textbf{C}\cdid}~and {\rm \textbf{C}\cdit}]
  Let $A$ be a formula. Proof-search for the sequent $\Rightarrow A$ in {\rm \textbf{C}\cdid}~and {\rm \textbf{C}\cdit}~terminates with a finite derivation in which either all the leaves are axiomatic or there is at least one global-saturated leaf.
\end{theorem}
